Evaluating and Mitigating Linguistic Discrimination in Large Language Models

By training on text in various languages, large language models (LLMs) typically possess multilingual support and demonstrate remarkable capabilities in solving tasks described in different languages. However, LLMs can exhibit linguistic discrimination due to the uneven distribution of training data across languages. That is, LLMs are hard to keep the consistency of responses when faced with the same task but depicted in different languages. In this study, we first explore the consistency in the LLMs' outputs responding to queries in various languages from two aspects: safety and quality. We conduct this analysis with two datasets (AdvBench and NQ) based on four LLMs (Llama2-13b, Gemma-7b, GPT-3.5-turbo and Gemini-pro). The results show that LLMs exhibit stronger human alignment capabilities with queries in English, French, Russian, and Spanish (only 1.04\% of harmful queries successfully jailbreak on average) compared to queries in Bengali, Georgian, Nepali and Maithili (27.7\% of harmful queries jailbreak successfully on average). Moreover, for queries in English, Danish, Czech and Slovenian, LLMs tend to produce responses with a higher quality (with 0.1494 $F_1$ score on average) compared to the other languages. Upon these findings, we propose LDFighter, a similarity-based voting, to mitigate the linguistic discrimination in LLMs. LDFighter ensures consistent service for different language speakers. We evaluate LDFighter with both benign queries and harmful queries. The results show that LDFighter not only significantly reduces the jailbreak success rate but also improve the response quality on average, demonstrating its effectiveness.

==> section4_copy.tex <==
\section{Mitigation of linguistic discrimination}
\label{sec:4}
Based on the above findings, in this section, we introduce LDFighter, a lightweight approach designed to mitigate linguistic discrimination from both safety and quality perspectives. LDFighter involves several steps. First, a query is translated into a selection of $K$ languages. Then, each translated query is inputted into a target LLM to generate responses in different languages. Next, these responses are translated to English, and the average similarity of each response to others are calculated. Finally, the response with the highest average similarity is selected as the final answer to the original query. Note that the selected answer will be translated back into the language of the original query if required. In the following, we introduce how the similarity-based voting works for the response, and then assess the effectiveness of LDFighter based on three research questions. 

\subsection{Similarity-based Voting}
% A straightforward way to eliminate the linguistic discrimination is to focus on one language. That is, we can translate the response in one high-resource language such as English to the language of the input query. However, relying on single language may suffer the safety problem because existing adversarial prompts and jailbreaking approaches mainly focus on certain languages. (need additonal experiments...)
Intuitively, when presented with the same question, different individuals tend to offer answers that exhibit certain similarities (assuming they possess similar ground-truth knowledge). Inspired by this observation, we select the response most similar to others from a set of responses as the final output of the target LLM. To achieve this, we adopt a cosine similarity to measure the similarity between pairs of responses. 

Algorithm~\ref{alg:sm} details the process for generating a response using similarity-based voting. Given a set of responses $\mathcal{R}$ in English translated from different languages, each response is first encoded into a vector, resulting in a set of vectors $\mathcal{V}$ (line 1). Next, the average similarity of each vector to the other vectors is calculated according to Formula~\ref{fm:sm} (lines 2-5), and the vector with the highest average similarity is chosen (line 6). Finally, the response corresponding to the selected vector is returned as the final response of the LLM.
\begin{algorithm}[t]
    \caption{$vote(\mathcal{R})$}
    \label{alg:sm}
    $\mathcal{V} \leftarrow$ encode each response $r\in R$\;
    let $\Gamma$ be an empty set\;
    \For{each answer $v \in \mathcal{V}$}{
        $s \leftarrow avgCos(\mathcal{V})$ \;
        $\Gamma \leftarrow \Gamma \cup \{s\} $\;
    }
    $\hat{v} \leftarrow max(\Gamma)$\;
    $r \leftarrow$ response responding to $\hat{v}$\;
    \Return{r}\;
\end{algorithm}

\begin{align}
    avgCos(\mathcal{V}) = \frac{\sum_{j\neq k}Cos(v_k,v_j)}{|\mathcal{V}|-1}
    \label{fm:sm}
\end{align}
% 1. safety
% 2. quality
\subsection{Research Questions}
In the following, we evaluate the effectiveness of LDFighter by addressing three key research questions.
\begin{itemize}
    \item RQ4: How effective is LDFighter on improving the safety performance of LLMs across different languages?
    \item RQ5: How effective is LDFighter on improving the response quality of LLMs across different languages?
    \item RQ6: What is the cost of LDFighter?
\end{itemize}
LLMs equipped with LDFighter inherently offer consistent service across all languages. In addition to ensuring consistency, we investigate whether LDFighter can maintain or surpass the original performance of LLMs in terms of safety and quality. Therefore, RQ4 and RQ5 aim to assess LDFighter's effectiveness in improving multilingual safety performance and response quality, respectively. RQ6 evaluates the time efficiency of LDFighter. We adopt the state-of-the-art text embedding model SFR-Embedding-Mistral~\cite{SFRAIResearch2024,muennighoff2022mteb} to encode each response. All the experiments are conducted on a cloud server equipped with two RTX 4090D (24GB), a 36 vCPU AMD EPYC 9754 128-core processor and 120 GB RAM, running on Ubuntu 20.04.5 LTS(64 bit).
\subsection{Results}
\begin{figure*}[t] 
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/mjr_vote.pdf}
        \caption{MJR of different LLMs with LDFighter}
        \label{fig:mjr_vote}
    \end{minipage} 
    \hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/f1_vote.pdf} 
        \caption{$F_1$-score of different LLMs with LDFighter}
        \label{fig:f1_vote}
    \end{minipage}
\end{figure*}
\noindent\emph{\textbf{RQ4: How effective is LDFighter on improving the safety performance of LLMs across different languages?}} To answer this question, we apply LDFighter to AdvBench and report the MJR of each LLMs. For each LLM, we select the top three languages with the highest CI scores. To investigate the impact of the number of languages on MJR, we vary the number of languages $K$ from 3 to 30 with step 3. Additionally, we examine the performance of LDFighter when using only one language, i.e., English, to determine if using multiple languages is necessary. 

Figure~\ref{fig:mjr_vote} shows the MJR of four LLMs without or with the help of LDFighter. The values responding to ``ori'' on x-axis are the result of each LLM without LDFighter, the values responding to ``eng'' are the result of each LLM with LDFighter where only one language, i.e., English, is used. When the value of $k$ is set to be 3 or above, the MJR of each LLM drops significantly compared to the original MJR.  Particularly, the MJR of GPT-3.5, Gemini-pro and Llama2-13b falls straight to 0.0 when using the top three languages, and then remain unchanged as $k$ increases. For Gemma-7b, the MJR first decreases to the lowest point at $k=3$, then rises slightly and stabilizes around 0.1 after $k=18$. When using only English in LDFighter, only Llama2-13b achieves an MJR of 0.0, while the other three LLMs do not reach their optimal MJR. Based on these experimental results, we can answer RQ4 as follows.
\begin{framed}
    \noindent \emph{Answer to RQ4: LDFighter demonstrates significant effectiveness in reducing the jailbreak rate of harmful questions. Moreover, the use of three languages with the highest CI leads to the lowest MJR for three out of the four LLMs.} 
\end{framed}
\noindent\emph{\textbf{RQ5: How effective is LDFighter on improving the response quality of LLMs across different languages?}} To answer this question, we apply LDFighter to the NQ dataset and evaluate the average $F_1$-score of four LLMs. The top-k settings are consistent with RQ4.

Figure~\ref{fig:f1_vote} illustrates the average $F_1$-score of four LLMs, both with and without LDFighter. Compared to the original average $F_1$-score, all LLMs experience an increase in average $F_1$-score with LDFighter, though the extent varies. For GPT-3.5 and Gemini-pro, the average $F_1$-score rises significantly and peaks when using only English in LDFighter. As $k$ continues to increase, the average $F_1$-score slightly decreases but still remains higher than the original average. For Gemma-7b and Llama2-13b, the average $F_1$-score steadily improves at first, reaching its maximum at $k=12$ for Gemma-7b and K=3 for Llama2-13b, after which it stabilizes. We thus have the following answer to RQ5.
\begin{framed}
    \noindent \emph{Answer to RQ5: LDFighter substantially enhances the average $F_1$-score of responses across four LLMs, indicating its potential to improve response quality for speakers of different languages.}
\end{framed}
\noindent\emph{\textbf{RQ6: What is the time overhead of LDFighter?}} The time overhead of LDFighter primarily consists of three parts: translation, querying, and encoding. Compared to the time spent interacting with LLMs, the time required for similarity-based voting can be considered negligible if the embeddings of each response have already been prepared. Let $t_{tra}$, $t_{qry}$, and $t_{emd}$ represent the time costs of translation, querying with an LLM, and sentence encoding, respectively. Therefore, the overall time cost of applying LDFighter can be estimated as follows:
\begin{align}
    cost = 2k \cdot t_{tra}+k\cdot t_{qry} + k \cdot t_{emd}
\end{align}
where $k$ is the number of languages used in LDFighter. The translation time is $2k \cdot t_{tra}$ because we need to translate both the original query and responses in different languages.

The time overhead varies linearly with the value of $k$, but it can be reduced by parallelizing the computation process of $k$ languages. We thus report the cost of LDFighter with k=1. On average, the time cost per query is 9.96 seconds on GPT-3.5, 4.91 seconds on Gemini-pro, 9.68 seconds on Gemma-7b, and 11.75 seconds on Llama2-13b. We thus have the following answer to RQ6.
\begin{framed}
    \noindent \emph{Answer to RQ6: LDFighter has the potential to be applied at runtime.}
\end{framed}
We remark that indeed there is additional token-cost when close-source API such as ChatGPT is adopted. However, such cost can be effectively mitigated if we adopt LDFighter with only English. 
